AugTriever: Unsupervised Dense Retrieval and Domain Adaptation by Scalable Data Augmentation

Dense retrievers have made significant strides in text retrieval and open-domain question answering. However, most of these achievements have relied heavily on extensive human-annotated supervision. In this study, we aim to develop unsupervised methods for improving dense retrieval models. We propose two approaches that enable annotation-free and scalable training by creating pseudo querydocument pairs: query extraction and transferred query generation. The query extraction method involves selecting salient spans from the original document to generate pseudo queries. On the other hand, the transferred query generation method utilizes generation models trained for other NLP tasks, such as summarization, to produce pseudo queries. Through extensive experimentation, we demonstrate that models trained using these augmentation methods can achieve comparable, if not better, performance than multiple strong dense baselines. Moreover, combining these strategies leads to further improvements, resulting in superior performance of unsupervised dense retrieval, unsupervised domain adaptation and supervised finetuning, benchmarked on both BEIR and ODQA datasets. Code and datasets are publicly available at https://github.com/salesforce/AugTriever.

==> table-fullscore.tex <==
\clearpage
\eject \pdfpagewidth=58cm \pdfpageheight=39cm
\thispagestyle{empty}

\begin{table*}[!ht]
\centering
\begin{minipage}{0.9\pdfpagewidth}
\renewcommand{\arraystretch}{0.5}
% \footnotesize
\tiny
\begin{adjustbox}{width=1\textwidth}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{tabular}{llcccccccccccccccgccccccccccccccccccggg}
\toprule
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \multicolumn{3}{c}{NQ} & \multicolumn{3}{c}{TriviaQA} & \multicolumn{3}{c}{WQ} & \multicolumn{3}{c}{CuratedTREC} & \multicolumn{3}{c}{SQuAD v1.1} & \multicolumn{3}{c}{EQ (Macro-Avg)} & \multicolumn{3}{c}{Average} \\\cmidrule{19-39}
\multicolumn{1}{l}{\multirow{-2}{*}{\textbf{Setting}}} & \multicolumn{1}{l}{\multirow{-2}{*}{\textbf{Model}}} & \multicolumn{1}{c}{\multirow{-2}{*}{MS MARCO}} & \multicolumn{1}{c}{\multirow{-2}{*}{TREC-COVID}} & \multicolumn{1}{c}{\multirow{-2}{*}{NFCorpus}} & \multicolumn{1}{c}{\multirow{-2}{*}{NQ}} & \multicolumn{1}{c}{\multirow{-2}{*}{HotpotQA}} & \multicolumn{1}{c}{\multirow{-2}{*}{FiQA-2018}} & \multicolumn{1}{c}{\multirow{-2}{*}{ArguAna}} & \multicolumn{1}{c}{\multirow{-2}{*}{Tóuche-2020}} & \multicolumn{1}{c}{\multirow{-2}{*}{DBPedia}} & \multicolumn{1}{c}{\multirow{-2}{*}{SCIDOCS}} & \multicolumn{1}{c}{\multirow{-2}{*}{FEVER}} & \multicolumn{1}{c}{\multirow{-2}{*}{Climate-FEVER}} & \multicolumn{1}{c}{\multirow{-2}{*}{SciFact}} & \multicolumn{1}{c}{\multirow{-2}{*}{Quora}} & \multicolumn{1}{c}{\multirow{-2}{*}{CQADupStack}} & \multirow{-2}{*}{BEIR Avg (14)} & {R@5} & {R@20} & {R@100} & {R@5} & {R@20} & {R@100} & {R@5} & {R@20} & {R@100} & {R@5} & {R@20} & {R@100} & {R@5} & {R@20} & {R@100} & {R@5} & {R@20} & {R@100} & {R@5} & {R@20} & {R@100} \\\midrule\midrule
\textbf{Baselines}\\
\midrule
 & BM25 & \textbf{22.8} & \bestcell\textbf{65.6} & 32.5 & \textbf{32.9} & \bestcell\textbf{60.3} & 23.6 & 31.5 & \bestcell\textbf{36.7} & \textbf{31.3} & 15.8 & \bestcell\textbf{75.3} & \secbestcell\textbf{21.3} & 66.5 & 78.9 & \secbestcell\textbf{29.9} & \bestcell\textbf{43.0} & 43.8 & 63.0 & 78.2 & 66.3 & 76.4 & 83.1 & 41.8 & 62.3 & 75.5 & 64.6 & 81.1 & 90.4 & \bestcell57.5 & 71.2 & 82.0 & \secbestcell61.0 & \bestcell71.4 & \bestcell80.1 & 55.8 & 70.9 & 81.5 \\
 & Contriever $\dagger$ & 20.6 & 27.5 & 31.7 & 25.4 & 48.1 & 24.5 & 37.9 & 16.7 & 29.2 & 14.9 & \secbestcell\textbf{68.2} & 15.5 & 64.9 & \bestcell\textbf{83.5} & 28.4 & 36.9 & 47.2 & 67.2 & 81.3 & 59.5 & 74.2 & 83.2 & 44.0 & 65.8 & 79.8 & 67.7 & 85.5 & 93.1 & 44.2 & 63.1 & 78.4 & 50.3 & 64.7 & 76.3 & 52.1 & 70.1 & 82.0 \\
 & SPAR $\dagger$ & 19.3 & 53.1 & 26.5 & 26.2 & 57.2 & 18.5 & 42.0 & 23.4 & 28.1 & 13.4 & 56.9 & 16.4 & 62.7 & 70.4 & 27.9 & 37.3 & 43.9 & 61.8 & 76.8 & 64.4 & 75.5 & 83.1 & 40.7 & 59.9 & 74.7 & 62.5 & 79.1 & 90.4 & 52.1 & 67.1 & 79.2 & 57.4 & 68.2 & 77.7 & 53.5 & 68.6 & 80.3 \\
 & Spider $\dagger$ & 15.0 & 32.2 & 26.7 & 14.5 & 41.3 & 9.1 & 29.0 & 4.7 & 21.6 & 13.0 & 31.6 & 12.9 & 62.3 & 72.4 & 22.2 & 28.1 & 48.3 & 67.6 & 80.8 & 63.4 & 75.4 & 83.4 & 45.5 & 65.8 & 80.1 & 64.7 & 83.4 & 93.1 & 43.9 & 61.8 & 77.0 & 53.0 & 65.3 & 76.9 & 53.1 & 69.9 & 81.9 \\
 & CPT-text S & & 52.9 & 32.0 & & 51.5 & 34.1 & 38.7 & 21.0 & 27.2 & & 57.1 & 15.8 & 65.4 & 68.1 & &  & & & & & & & & & & & & & & & & & & & & & \\
 & CPT-text M & & 44.3 & 34.5 & & 53.0 & \secbestcell37.3 & 41.2 & 23.3 & 29.6 & & 58.2 & 15.6 & 68.3 & 70.3 & &  & & & & & & & & & & & & & & & & & & & & & \\
 & CPT-text L & & 42.7 & \bestcell\textbf{36.9} & & 54.3 & \bestcell\textbf{39.7} & 39.2 & 22.8 & 31.2 & & 63.8 & 16.1 & \bestcell\textbf{71.2} & 68.7 & &  & & & & & & & & & & & & & & & & & & & & & \\
 % & Spider & & & & & & & & & & & & & & & &  & {49.6} & {68.3} & {81.2} & {63.6} & {75.8} & {83.5} & {46.8} & {65.9} & {79.7} & {65.9} & {82.6} & {92.8} & {43.6} & {61.0} & {76.0} & {54.5} & {66.3} & {77.4} & 54.0 & 70.0 & 81.8 \\
 % & Spider+BM25 & & & & & & & & & & & & & & & &  & \textbf{55.1} & \textbf{72.1} & \textbf{84.1} & \textbf{71.7} & \textbf{80.0} & \textbf{85.5} & \textbf{51.0} & \textbf{69.1} & \textbf{81.1} & \textbf{74.5} & \textbf{86.5} & \textbf{93.9} & \textbf{60.9} & \textbf{74.6} & \textbf{84.5} & \textbf{65.4} & \textbf{75.0} & \textbf{82.6} & \textbf{63.1} & \textbf{76.2} & \textbf{85.3} \\
 & Condenser & & & & & & & & & & & & & & & &  & {13.0} & {25.5} & {43.4} & {4.5} & {9.6} & {18.5} & {20.3} & {35.8} & {51.9} & {9.9} & {20.2} & {34.4} & {6.1} & {13.2} & {25.3} & {1.0} & {2.7} & {7.6} & 9.1 & 17.8 & 30.2 \\
 & CoCondenser & & & & & & & & & & & & & & & &  & {28.9} & {46.8} & {63.5} & {7.5} & {13.8} & {24.3} & {30.2} & {50.7} & {68.7} & {11.7} & {22.5} & {39.3} & {8.5} & {16.5} & {28.8} & {0.5} & {1.4} & {8.7} & 14.6 & 25.3 & 38.9 \\

\midrule \midrule 
\textbf{Pile-CC} &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule 
RC & Inbatch & 16.3 & 28.7 & 20.8 & 15.5 & 34.4 & 15.2 & 43.9 & 4.6 & 20.5 & 9.6 & 22.6 & 7.9 & 56.7 & 81.4 & 22.3 & 27.4 & 45.4 & 65.2 & 78.5 & 57.5 & 72.2 & 81.9 & 52.0 & 70.1 & 81.3 & 66.4 & 85.0 & 92.9 & 42.0 & 60.6 & 75.2 & 40.7 & 54.8 & 69.3 & 50.7 & 68.0 & 79.8 \\
RC & MoCo & 19.2 & 39.5 & 28.0 & 22.3 & 43.0 & 21.2 & 38.1 & 12.6 & 22.2 & 13.8 & 48.1 & 14.6 & 63.5 & 81.8 & 27.1 & 34.0 & 44.7 & 64.2 & 78.1 & 59.2 & 73.8 & 82.5 & 45.3 & 65.6 & 80.6 & 63.4 & 82.4 & 93.2 & 43.0 & 62.5 & 77.2 & 47.6 & 61.3 & 73.8 & 50.5 & 68.3 & 80.9 \\
QGen-D2Q & Inbatch & 24.4 & 55.9 & 31.6 & \textbf{35.5} & 53.2 & \textbf{29.8} & 33.8 & 16.5 & 32.1 & 15.3 & 62.3 & 14.2 & 60.8 & 80.7 & \bestcell\textbf{30.6} & 39.5 & \textbf{51.8} & \textbf{72.1} & \textbf{84.4} & 60.2 & 74.6 & 83.5 & 46.7 & 68.9 & 81.6 & 70.0 & 87.0 & \textbf{94.5} & 39.2 & 58.2 & 73.5 & 55.7 & 68.3 & 77.9 & 53.9 & 71.5 & 82.6 \\
QGen-D2Q+RC & MoCo & 23.2 & \textbf{63.4} & 31.5 & 32.5 & 52.4 & 28.0 & 38.1 & \textbf{20.5} & 29.4 & 14.8 & 55.1 & 14.2 & 65.9 & 81.9 & 29.7 & 39.8 & 51.7 & 70.6 & 82.8 & 63.6 & 76.3 & 83.8 & \textbf{52.9} & \textbf{71.5} & \textbf{82.4} & \textbf{70.8} & \textbf{87.9} & 94.0 & 43.8 & 63.3 & 77.9 & 55.3 & 67.9 & 78.3 & \textbf{56.3} & \textbf{72.9} & 83.2 \\

\hdashline\\
% Hybrid-All & MoCo & 23.3 & 58.0 & 30.5 & 28.4 & 53.5 & 25.1 & 39.2 & 17.8 & 31.8 & 15.6 & 62.1 & 17.0 & 63.3 & 77.4 & 26.5 & 43.3 & 56.7 & 66.1 & 80.4 & 70.3 & 75.7 & 83.6 & 60.5 & 69.7 & 81.9 & 78.0 & 85.7 & 92.9 & 53.2 & 62.3 & 77.3 & 61.0 & 66.5 & 77.8 & 63.3 & 71.0 & 82.3 \\
% Hybrid-TQGen & MoCo & 23.5 & 58.5 & 30.3 & 28.9 & 53.6 & 25.2 & 38.0 & 19.6 & 32.3 & 15.3 & 61.4 & 17.5 & 65.2 & 78.7 & 26.5 & 43.7 & 57.3 & 66.4 & 80.7 & 70.3 & 75.6 & 83.7 & 60.3 & 69.4 & 82.2 & 79.3 & 85.2 & 93.2 & 53.2 & 62.4 & 77.7 & 60.3 & 66.5 & 77.3 & 63.4 & 70.9 & 82.5 \\
% Hybrid-TQGen+ & MoCo & \textbf{24.6} & 59.5 & 32.7 & 32.7 & \textbf{57.1} & 26.9 & 41.2 & 17.8 & \textbf{32.6} & \textbf{16.8} & \textbf{65.5} & 16.4 & \textbf{67.8} & 79.3 & 29.4 & \textbf{45.2} & 60.3 & 69.7 & 82.7 & 71.3 & 76.6 & 84.3 & 62.7 & 70.7 & 82.3 & 81.6 & 86.9 & 93.4 & 54.6 & 63.4 & 78.0 & 63.4 & 68.5 & 78.7 & 65.6 & 72.6 & 83.3 \\

Hybrid-All & MoCo & 23.3 & 58.0 & 30.5 & 28.4 & 53.5 & 25.1 & 39.2 & 17.8 & 31.8 & 15.6 & 62.1 & 17.0 & 63.3 & 77.4 & 26.5 & 39.4 & 46.0 & 66.4 & 80.7 & 63.0 & 75.6 & 83.7 & 48.7 & 69.4 & 82.2 & 68.0 & 85.2 & 93.2 & 43.1 & 62.4 & 77.7 & 53.5 & 66.5 & 77.3 & 53.7 & 70.9 & 82.5 \\
Hybrid-TQGen & MoCo & 23.5 & 58.5 & 30.3 & 28.9 & 53.6 & 25.2 & 38.0 & 19.6 & 32.3 & 15.3 & 61.4 & 17.5 & 65.2 & 78.7 & 26.5 & 39.0 & 45.6 & 66.1 & 80.4 & 62.8 & 75.7 & 83.6 & 49.0 & 69.7 & 81.9 & 67.0 & 85.7 & 92.9 & 42.5 & 62.3 & 77.3 & 53.6 & 66.5 & 77.8 & 53.4 & 71.0 & 82.3 \\
Hybrid-TQGen+ & MoCo & \secbestcell\textbf{24.6} & 59.5 & 32.7 & 32.7 & 57.1 & 26.9 & 41.2 & 17.8 & \secbestcell\textbf{32.6} & \bestcell\textbf{16.8} & \textbf{65.5} & 16.4 & 67.8 & 79.3 & 29.4 & 41.1 & 49.5 & 69.7 & 82.7 & \textbf{64.1} & \textbf{76.6} & \textbf{84.3} & 51.1 & 70.7 & 82.3 & 69.9 & 86.9 & 93.4 & 43.9 & 63.4 & 78.0 & \textbf{56.6} & \textbf{68.5} & \textbf{78.7} & 55.8 & 72.6 & \textbf{83.3} \\

Hybrid-TQGen++ & MoCo & \bestcell \textbf{25.4} & \textbf{64.0}  & \secbestcell \textbf{35.1}  & 33.5  & \secbestcell\textbf{57.6} & 29.2   & 39.8   & 19.8   & \bestcell\textbf{32.7}  & \secbestcell\textbf{16.7}  & 65.3   & 15.9  & \secbestcell \textbf{68.7} & 79.9  & \bestcell\textbf{30.6}  & \secbestcell\textbf{42.1}
& 50.2 & 70.0 & 83.1 & \textbf{65.4} & \textbf{77.2} & \textbf{84.5} & 50.5 & 70.6 & 82.3 & \textbf{72.8} & 86.9 & 93.8 & 44.7 & \textbf{64.2} & 78.4 & \textbf{58.2} & \textbf{69.9} & \textbf{79.2} & \textbf{57.0} & \textbf{73.1} & \textbf{83.6}\\

\\\hdashline\\



Doc-Title & Inbatch & 19.7 & 35.1 & 27.6 & 27.2 & 44.5 & 22.1 & 24.6 & 9.8 & 30.3 & 14.2 & 56.4 & 12.0 & 59.4 & 79.7 & 22.4 & 33.2 & 46.7 & 66.4 & 80.8 & 58.7 & 72.8 & 82.4 & 47.3 & 68.9 & 81.3 & 67.0 & 86.0 & 93.1 & 38.6 & 57.3 & 73.1 & 47.9 & 62.1 & 74.4 & 51.0 & 68.9 & 80.8 \\
Doc-Title+RC & MoCo & 21.8 & 55.3 & 29.7 & 28.9 & 51.2 & 25.3 & 37.9 & 18.4 & 31.0 & 15.8 & 59.1 & 17.1 & 63.5 & 81.3 & 28.0 & 38.7 & 46.9 & 67.5 & 80.1 & 62.3 & 75.9 & 83.7 & 50.7 & 70.5 & 81.9 & 70.5 & 85.2 & 93.5 & \textbf{44.9} & \textbf{64.0} & 77.9 & 51.0 & 64.5 & 76.0 & 54.4 & 71.3 & 82.2 \\\\
QExt-BM25 & Inbatch & 16.3 & 27.2 & 21.6 & 17.1 & 34.3 & 16.6 & 40.5 & 5.3 & 20.1 & 10.3 & 26.0 & 8.1 & 56.4 & 81.4 & 24.2 & 27.8 & 46.5 & 66.1 & 79.5 & 58.1 & 72.5 & 82.1 & 51.1 & 70.0 & 81.6 & 68.4 & 85.6 & 93.2 & 41.8 & 60.7 & 75.8 & 42.1 & 56.0 & 70.3 & 51.3 & 68.5 & 80.4 \\
QExt-BM25+RC & MoCo & 20.2 & 46.8 & 28.4 & 24.3 & 47.5 & 22.6 & 37.2 & 13.3 & 25.2 & 14.6 & 53.0 & 16.1 & 63.0 & \secbestcell\textbf{82.7} & 27.0 & 35.8 & 44.5 & 65.0 & 80.3 & 60.3 & 74.1 & 82.8 & 44.4 & 68.0 & 80.9 & 65.0 & 85.2 & 92.8 & 43.8 & 63.5 & 77.7 & 50.6 & 63.9 & 75.4 & 51.4 & 69.9 & 81.6 \\\\
QExt-PLM & Inbatch & 16.2 & 27.9 & 21.4 & 15.9 & 33.9 & 15.1 & \secbestcell\textbf{44.0} & 4.7 & 19.7 & 9.5 & 22.8 & 7.4 & 54.9 & 81.5 & 22.4 & 27.2 & 46.4 & 65.6 & 79.6 & 58.1 & 72.7 & 82.1 & 51.2 & 69.9 & 81.2 & 67.0 & 85.6 & 93.7 & 42.2 & 60.9 & 75.7 & 40.9 & 54.9 & 68.9 & 51.0 & 68.3 & 80.2 \\
QExt-PLM+RC & MoCo & 20.6 & 53.6 & 30.3 & 27.2 & 47.9 & 22.3 & 39.1 & 19.0 & 29.0 & 14.7 & 59.7 & 17.7 & 64.5 & \secbestcell\textbf{82.7} & 27.1 & 38.2 & 45.2 & 65.2 & 79.9 & 61.3 & 74.8 & 83.3 & 45.7 & 68.1 & 81.4 & 65.6 & 84.0 & 93.1 & 44.7 & 63.7 & \textbf{78.7} & 50.9 & 64.4 & 76.3 & 52.2 & 70.0 & 82.1 \\\\
TQGen-Topic & Inbatch & 20.7 & 58.2 & \textbf{34.1} & 27.6 & 49.4 & 28.1 & 36.7 & 18.6 & 31.2 & 16.0 & 63.9 & 12.1 & 61.8 & 78.5 & 30.3 & 39.0 & 44.2 & 65.0 & 80.3 & 56.9 & 72.3 & 82.3 & 41.0 & 65.2 & 80.6 & 63.5 & 83.7 & 92.7 & 37.1 & 57.1 & 73.8 & 49.4 & 64.0 & 75.7 & 48.7 & 67.9 & 80.9 \\
TQGen-Topic+RC & MoCo & 21.2 & 61.6 & 30.7 & 27.4 & 51.7 & 24.7 & 40.0 & 17.3 & 30.7 & 15.8 & 59.6 & 14.7 & 64.8 & 77.9 & 27.9 & 38.9 & 45.6 & 65.7 & 80.9 & 62.0 & 75.4 & 83.7 & 45.7 & 67.3 & 81.1 & 67.2 & 84.9 & 93.5 & 42.2 & 62.3 & 77.6 & 50.7 & 64.5 & 76.4 & 52.2 & 70.0 & 82.2 \\\\
TQGen-Title & Inbatch & 20.0 & 46.5 & 32.1 & 28.9 & 49.6 & 27.0 & 32.9 & 14.3 & 30.9 & 16.4 & 64.2 & 14.1 & 62.7 & 80.1 & 29.6 & 37.8 & 44.7 & 65.7 & 80.5 & 57.5 & 73.2 & 82.7 & 42.2 & 66.7 & 80.9 & 64.7 & 84.3 & 92.8 & 36.2 & 56.0 & 72.5 & 49.8 & 64.0 & 75.7 & 49.2 & 68.3 & 80.8 \\
TQGen-Title+RC & MoCo & 21.8 & 60.0 & 31.0 & 29.0 & 51.8 & 26.3 & 39.3 & 17.0 & 30.0 & 15.8 & 60.7 & 16.1 & 65.0 & 79.4 & 28.7 & 39.3 & 46.8 & 66.6 & 80.4 & 62.7 & 75.8 & 83.9 & 48.2 & 69.0 & 82.0 & 66.0 & 85.3 & 92.9 & 42.4 & 62.2 & 77.1 & 52.8 & 66.2 & 77.2 & 53.1 & 70.8 & 82.3 \\\\
TQGen-AbSum & Inbatch & 18.1 & 39.8 & 29.5 & 26.7 & 45.5 & 25.7 & 33.5 & 13.6 & 30.0 & 15.6 & 54.1 & 12.9 & 60.0 & 79.6 & 28.2 & 35.3 & 43.5 & 64.5 & 79.7 & 55.9 & 72.4 & 82.1 & 45.1 & 67.1 & 80.3 & 64.1 & 84.0 & 92.8 & 35.3 & 54.8 & 71.8 & 45.7 & 60.0 & 72.9 & 48.3 & 67.1 & 79.9 \\
TQGen-AbSum+RC & MoCo & 23.3 & 52.7 & 29.9 & 29.8 & 54.0 & 26.8 & 38.7 & 20.2 & 31.1 &16.6 & 63.6 & \textbf{17.8} & 65.6 & 78.1 & 29.3 & 39.6 & 48.3 & 67.1 & 81.0 & 62.3 & 75.6 & 83.9 & 48.7 & 69.7 & 81.4 & 68.3 & 85.3 & 92.8 & 43.6 & 62.3 & 77.0 & 55.0 & 67.4 & 77.8 & 54.4 & 71.2 & 82.3 \\\\
TQGen-ExSum & Inbatch & 18.9 & 40.5 & 30.4 & 27.4 & 46.7 & 26.9 & 34.3 & 13.9 & 31.3 & 15.1 & 55.9 & 13.4 & 62.2 & 80.6 & 29.1 & 36.3 & 46.0 & 66.5 & 81.0 & 56.5 & 73.1 & 82.4 & 45.4 & 67.5 & 79.7 & 64.8 & 84.2 & 92.1 & 36.4 & 55.8 & 72.4 & 47.3 & 61.5 & 73.8 & 49.4 & 68.1 & 80.2 \\
TQGen-ExSum+RC & MoCo & 23.0 & 55.8 & 29.4 & 29.5 & 54.4 & 27.6 & 39.4 & 16.3 & 31.8 & 16.1 & 61.2 & 16.4 & 65.6 & 79.0 & 28.7 & 39.4 & 48.8 & 67.9 & 80.8 & 63.2 & 76.1 & 83.8 & 49.4 & 69.8 & 81.5 & 67.2 & 85.3 & 92.5 & 43.6 & 63.0 & 77.7 & 54.2 & 66.8 & 77.5 & 54.4 & 71.5 & 82.3 \\
 
 \midrule\midrule
\textbf{Wikipedia} &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
RC & Inbatch & 14.0 & 23.8 & 13.7 & 20.2 & 32.0 & 9.4 & 43.2 & 2.9 & 19.2 & 8.1 & 23.3 & 10.8 & 52.4 & 76.8 & 18.1 & 25.3 & 40.7 & 60.3 & 75.7 & 50.9 & 66.9 & 79.1 & 30.2 & 50.7 & 68.7 & 48.3 & 69.6 & 86.9 & 29.4 & 49.6 & 67.9 & 26.4 & 40.3 & 58.4 & 37.6 & 56.2 & 72.8 \\
RC & MoCo & 17.5 & 35.5 & 22.8 & 25.1 & 42.1 & 13.8 & 38.5 & 6.9 & 22.0 & 12.1 & 40.5 & 15.7 & 60.9 & 76.7 & 20.8 & 30.9 & 43.8 & 62.9 & 77.5 & 55.8 & 70.7 & 80.8 & 30.2 & 52.2 & 70.9 & 48.6 & 72.6 & 88.6 & 34.0 & 53.4 & 71.4 & 36.6 & 51.7 & 67.5 & 41.5 & 60.6 & 76.1 \\\\

QGen-D2Q & Inbatch & \bestcell\textbf{25.4} & 58.3 & 26.1 & \secbestcell39.8 & 55.3 & \textbf{23.6} & 28.9 & 17.2 & 31.0 & 11.7 & 67.9 & \bestcell\textbf{21.7} & 59.2 & 77.7 & 20.4 & 38.5 & 58.2 & 75.5 & 86.1 & 65.0 & 76.7 & 83.6 & \secbestcell56.7 & \bestcell\textbf{73.8} & \secbestcell82.7 & 75.7 & 88.6 & 93.8 & 44.3 & 62.5 & 76.8 & \bestcell\textbf{61.7} & \bestcell\textbf{71.7} & \secbestcell\textbf{79.8} & 60.3 & 74.8 & 83.8 \\
QGen-D2Q+RC & Inbatch & 23.5 & 53.1 & 22.7 & 39.6 & 54.5 & 22.5 & 41.0 & 14.7 & 27.3 & 10.9 & 44.0 & 13.1 & 60.0 & 62.9 & 22.8 & 34.9 & 57.8 & 74.9 & 85.5 & 65.6 & 77.0 & 84.1 & 56.0 & 73.5 & 82.3 & 75.9 & 88.0 & 94.0 & 46.7 & 63.9 & 77.5 & 60.3 & 70.7 & 79.4 & 60.4 & 74.7 & 83.8 \\
QGen-D2Q & MoCo & 16.3 & 42.5 & 19.7 & 19.8 & 38.0 & 12.3 & 32.5 & 8.3 & 25.1 & 9.7 & 26.6 & 10.9 & 46.4 & 75.3 & 17.7 & 27.5 & 39.4 & 59.0 & 74.9 & 57.6 & 71.3 & 80.8 & 48.9 & 67.5 & 79.9 & 70.2 & 86.2 & 93.1 & 38.6 & 57.3 & 73.9 & 45.5 & 59.7 & 73.0 & 50.0 & 66.8 & 79.3 \\
QGen-D2Q+RC & MoCo & 23.7 & \secbestcell\textbf{64.9} & 26.2 & 35.9 & 55.3 & 22.1 & 36.8 & 21.1 & 28.1 & 12.8 & 50.3 & 17.9 & 62.3 & 79.9 & 25.4 & 38.5 & 53.8 & 71.8 & 83.4 & 66.0 & 77.4 & 84.1 & 54.7 & 71.6 & 82.5 & 76.1 & 88.8 & 94.5 & 47.1 & 65.8 & 79.4 & 56.4 & 69.0 & 78.9 & 59.0 & 74.0 & 83.8 \\\\

QGen-PAQ & Inbatch & 22.3 & 49.3 & 19.3 & \bestcell\textbf{42.6} & \textbf{55.9} & 16.4 & 2.0 & 12.8 & 24.1 & 10.3 & 42.2 & 10.5 & 55.0 & 74.0 & 20.1 & 31.0 & \bestcell\textbf{65.3} & \bestcell\textbf{79.7} & \bestcell\textbf{87.4} & \bestcell\textbf{72.5} & \bestcell\textbf{80.9} & \bestcell\textbf{86.0} & \bestcell\textbf{57.6} & \bestcell\textbf{73.8} & \bestcell\textbf{83.3} & \bestcell\textbf{82.1} & \bestcell\textbf{90.6} & \secbestcell95.7 & 55.2 & 71.2 & 82.4 & 59.8 & 70.5 & 79.4 & \bestcell\textbf{65.4} & \bestcell\textbf{77.8} & \bestcell\textbf{85.7} \\
QGen-PAQ+RC & Inbatch & 19.1 & 25.9 & 25.0 & 26.0 & 46.8 & 15.2 & 39.5 & 12.6 & 26.7 & 11.1 & 35.0 & 10.8 & 52.9 & 81.1 & 19.9 & 30.6 & 51.9 & 71.3 & 83.6 & 66.0 & 77.3 & 84.2 & 48.5 & 68.9 & 81.5 & 73.9 & 87.5 & 94.7 & 46.3 & 63.7 & 78.2 & 50.7 & 64.5 & 76.7 & 56.2 & 72.2 & 83.1 \\
QGen-PAQ & MoCo & 21.4 & 37.2 & 24.9 & 36.6 & 52.3 & 16.4 & 10.4 & 16.5 & 28.8 & 10.2 & 45.5 & 8.8 & 59.7 & 74.9 & 23.7 & 31.8 & \secbestcell63.4 & \secbestcell78.6 & \secbestcell87.1 & \secbestcell70.2 & \secbestcell80.3 & \secbestcell85.9 & 54.6 & \secbestcell72.2 & 82.6 & 79.1 & \secbestcell89.9 & 95.1 & \secbestcell\textbf{55.4} & \bestcell\textbf{71.9} & \secbestcell82.9 & 52.7 & 65.9 & 77.4 & \secbestcell62.6 & \secbestcell76.5 & \secbestcell85.2 \\
QGen-PAQ+RC & MoCo & 22.6 & 28.4 & 23.1 & 26.7 & 49.8 & 14.7 & 32.0 & 10.7 & 26.6 & 9.7 & 31.4 & 5.7 & 53.9 & \textbf{82.3} & 23.7 & 29.9 & 56.9 & 74.2 & 85.2 & 70.0 & 79.7 & 85.4 & 54.3 & 71.4 & 81.9 & 77.0 & 89.3 & \bestcell\textbf{96.1} & 55.1 & \secbestcell71.8 & \bestcell\textbf{83.0} & 52.6 & 66.0 & 77.7 & 61.0 & 75.4 & 84.9 \\

\hdashline
 &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
Doc-Title & Inbatch & 14.7 & 37.7 & 27.5 & 22.6 & 41.6 & 13.6 & 24.7 & 17.2 & 28.8 & 10.9 & 60.9 & 13.4 & 45.4 & 61.6 & 14.1 & 30.0 & 35.9 & 54.6 & 71.2 & 49.6 & 64.7 & 76.9 & 32.2 & 55.3 & 72.8 & 51.2 & 73.2 & 87.6 & 25.5 & 42.7 & 61.9 & 49.2 & 61.6 & 73.0 & 40.6 & 58.7 & 73.9 \\
Doc-Title+RC & Inbatch & 16.0 & 25.3 & 27.1 & 25.4 & 43.4 & 12.9 & 36.0 & 14.8 & 27.1 & 10.8 & 46.7 & 11.7 & 56.7 & 65.2 & 18.0 & 30.1 & 21.3 & 45.6 & 54.8 & 63.1 & 77.3 & 32.0 & 55.2 & 63.2 & 69.8 & \secbestcell80.7 & 12.9 & 32.7 & 44.1 & 53.0 & 71.4 & 23.3 & 51.3 & 62.3 & 71.0 & 87.3 & 12.4 \\
Doc-Title & MoCo & 12.0 & 42.3 & 23.0 & 14.5 & 34.7 & 7.1 & 31.9 & 8.0 & 22.9 & 10.1 & 19.7 & 4.6 & 47.7 & 72.4 & 14.3 & 25.2 & 32.3 & 51.6 & 68.9 & 48.3 & 63.9 & 76.3 & 34.3 & 53.3 & 72.2 & 51.7 & 71.3 & 85.7 & 26.1 & 44.3 & 63.1 & 39.6 & 53.2 & 67.0 & 38.7 & 56.3 & 72.2 \\
Doc-Title+RC & MoCo & 18.5 & 40.4 & 26.8 & 27.8 & 47.4 & 15.8 & 38.0 & 10.7 & 28.0 & 12.9 & 49.8 & 13.8 & 60.3 & 76.7 & 22.9 & 33.7 & 45.6 & 66.5 & 79.9 & 59.5 & 72.9 & 82.3 & 36.1 & 57.0 & 74.0 & 57.1 & 77.8 & 89.5 & 36.9 & 56.2 & 72.9 & 47.2 & 60.6 & 73.0 & 47.1 & 65.2 & 78.6 \\
 &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

Doc-Anchor & Inbatch & 15.6 & 36.3 & 27.1 & 22.3 & 44.6 & 12.5 & 26.3 & 13.7 & 26.9 & 11.6 & 42.7 & 10.1 & 50.0 & 74.5 & 18.3 & 29.8 & 36.4 & 56.7 & 74.3 & 55.7 & 70.6 & 80.8 & 32.7 & 55.6 & 74.4 & 51.6 & 76.5 & 89.3 & 28.9 & 47.9 & 67.6 & 35.9 & 51.8 & 68.2 & 40.2 & 59.9 & 75.8 \\
Doc-Anchor+RC & Inbatch & 16.5 & 32.3 & 27.7 & 22.4 & 38.9 & 14.1 & 34.1 & 9.5 & 25.7 & 12.6 & 21.2 & 11.0 & 60.7 & 76.7 & 20.8 & 29.1 & 41.7 & 61.9 & 77.6 & 57.3 & 71.3 & 81.9 & 31.9 & 51.9 & 72.6 & 52.0 & 75.4 & 88.3 & 31.6 & 50.6 & 69.7 & 31.4 & 46.1 & 63.1 & 41.0 & 59.5 & 75.5 \\
Doc-Anchor & MoCo & 16.7 & 49.5 & 25.6 & 23.5 & 49.6 & 14.1 & 38.0 & 14.6 & 29.1 & 12.8 & 40.5 & 13.6 & 54.2 & 76.8 & 20.9 & 33.1 & 39.4 & 58.7 & 75.9 & 59.5 & 73.1 & 82.1 & 36.2 & 57.2 & 76.0 & 60.1 & 79.1 & 91.6 & 37.5 & 55.8 & 72.7 & 44.1 & 58.4 & 72.2 & 46.1 & 63.7 & 78.4 \\
Doc-Anchor+RC & MoCo & 17.9 & 51.8 & 26.8 & 27.8 & 48.1 & 16.4 & 36.7 & 18.3 & 27.3 & 13.0 & 50.9 & 17.0 & 60.3 & 77.8 & 23.3 & 35.4 & 45.1 & 64.7 & 79.1 & 59.1 & 72.7 & 82.6 & 37.9 & 58.2 & 76.2 & 56.2 & 78.4 & 90.8 & 36.0 & 55.4 & 72.6 & 45.6 & 59.3 & 72.1 & 46.7 & 64.8 & 78.9 \\
 &  & & & & & & & & & & & & & & & &  & & & & & & & & & & & & & & & & & & & & & \\

QExt-Self & Inbatch & 11.4 & 30.2 & 16.4 & 19.1 & 39.0 & 11.8 & 8.8 & 2.3 & 12.6 & 9.5 & 37.2 & 14.1 & 59.6 & 71.2 & 19.9 & 25.1 & 39.3 & 56.8 & 72.7 & 48.5 & 64.2 & 77.2 & 28.7 & 47.6 & 66.5 & 46.8 & 68.2 & 83.4 & 31.0 & 48.7 & 66.3 & 29.1 & 42.9 & 59.7 & 37.2 & 54.7 & 71.0 \\
QExt-Self+RC & Inbatch & 14.6 & 25.9 & 15.6 & 22.1 & 36.0 & 11.3 & 36.7 & 3.5 & 20.8 & 9.0 & 32.5 & 13.2 & 54.7 & 77.2 & 20.2 & 27.1 & 41.5 & 60.3 & 75.8 & 51.5 & 67.1 & 79.4 & 29.8 & 50.6 & 68.1 & 47.6 & 71.2 & 86.2 & 31.5 & 50.7 & 69.6 & 26.7 & 40.3 & 58.8 & 38.1 & 56.7 & 73.0 \\
QExt-Self & MoCo & 9.9 & 29.1 & 16.1 & 14.0 & 28.1 & 9.1 & 2.2 & 4.4 & 18.7 & 8.0 & 18.7 & 10.8 & 38.4 & 69.3 & 14.9 & 20.1 & 34.7 & 51.4 & 67.6 & 48.7 & 64.1 & 76.7 & 34.6 & 54.7 & 71.7 & 54.3 & 75.2 & 88.2 & 32.0 & 50.0 & 67.6 & 29.9 & 43.0 & 58.5 & 39.0 & 56.4 & 71.7 \\
QExt-Self+RC & MoCo & 12.2 & 27.8 & 14.3 & 17.0 & 31.2 & 8.7 & 29.7 & 4.5 & 19.4 & 8.5 & 20.1 & 10.8 & 40.4 & 68.6 & 14.1 & 22.5 & 37.7 & 55.3 & 70.0 & 51.9 & 67.5 & 78.7 & 34.6 & 56.4 & 73.0 & 55.2 & 76.4 & 88.0 & 33.8 & 52.1 & 69.4 & 32.7 & 45.0 & 60.0 & 41.0 & 58.8 & 73.2 \\
 &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

QExt-BM25 & Inbatch & 11.4 & 30.2 & 16.4 & 19.1 & 39.0 & 11.8 & 8.8 & 2.3 & 12.6 & 9.5 & 37.2 & 14.1 & 59.6 & 71.2 & 19.9 & 25.1 & 39.2 & 58.0 & 73.5 & 49.9 & 66.2 & 78.4 & 27.8 & 47.7 & 65.9 & 44.7 & 67.0 & 83.7 & 28.1 & 46.6 & 65.7 & 30.6 & 45.0 & 62.1 & 36.7 & 55.1 & 71.5 \\
QExt-BM25+RC & Inbatch & 15.3 & 28.2 & 18.0 & 22.3 & 35.3 & 12.8 & 27.8 & 3.4 & 18.1 & 9.7 & 27.6 & 12.4 & 58.0 & 76.9 & 21.4 & 26.6 & 42.7 & 61.6 & 77.2 & 52.5 & 67.8 & 79.9 & 31.4 & 52.2 & 70.0 & 50.3 & 71.2 & 87.0 & 31.0 & 50.9 & 69.6 & 29.3 & 43.9 & 61.6 & 39.5 & 57.9 & 74.2 \\
QExt-BM25 & MoCo & 15.8 & 19.5 & 21.5 & 18.3 & 36.6 & 9.7 & 16.2 & 3.5 & 19.6 & 10.1 & 21.3 & 7.1 & 52.6 & 66.0 & 21.8 & 23.1 & 40.2 & 58.6 & 74.2 & 57.4 & 70.9 & 81.0 & 39.6 & 59.6 & 75.0 & 57.9 & 77.5 & 90.1 & 41.2 & 59.1 & 74.5 & 38.0 & 52.2 & 67.4 & 45.7 & 63.0 & 77.0 \\
QExt-BM25+RC & MoCo & 17.1 & 29.2 & 25.3 & 24.3 & 40.9 & 15.0 & 35.6 & 9.0 & 17.5 & 12.6 & 26.9 & 16.7 & 58.5 & 75.9 & 22.6 & 29.3 & 45.8 & 63.7 & 78.2 & 59.2 & 73.0 & 82.2 & 34.0 & 57.4 & 74.2 & 57.4 & 75.9 & 89.8 & 38.5 & 57.5 & 74.4 & 42.8 & 56.7 & 70.4 & 46.3 & 64.0 & 78.2 \\
 &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

QExt-PLM & Inbatch & 15.0 & 28.4 & 15.1 & 26.8 & 31.2 & 14.1 & 3.9 & 8.9 & 16.9 & 10.6 & 45.8 & 12.4 & 57.0 & 76.4 & 21.2 & 26.3 & 39.8 & 59.1 & 74.7 & 48.9 & 65.7 & 78.3 & 31.1 & 50.9 & 69.4 & 46.8 & 70.5 & 86.3 & 30.0 & 49.1 & 68.9 & 24.4 & 38.5 & 56.8 & 36.8 & 55.6 & 72.4 \\
QExt-PLM+RC & Inbatch & 15.1 & 28.0 & 21.8 & 25.0 & 34.8 & 12.8 & 11.1 & 8.1 & 21.6 & 10.4 & 39.7 & 13.8 & 57.1 & 77.1 & 21.8 & 27.4 & 40.9 & 59.9 & 75.3 & 49.4 & 66.1 & 79.1 & 29.5 & 49.9 & 69.2 & 47.0 & 70.9 & 86.6 & 29.6 & 49.7 & 69.1 & 23.1 & 37.6 & 56.9 & 36.6 & 55.7 & 72.7 \\
QExt-PLM & MoCo & 16.7 & 26.0 & 24.1 & 23.1 & 34.5 & 12.8 & \bestcell\textbf{44.5} & 11.9 & 22.3 & 11.5 & 26.7 & 10.6 & 57.4 & 78.6 & 21.3 & 29.0 & 43.6 & 62.5 & 77.5 & 58.8 & 72.6 & 81.8 & 37.1 & 59.2 & 76.7 & 59.4 & 79.7 & 91.6 & 38.2 & 57.6 & 74.5 & 42.9 & 57.3 & 71.6 & 46.6 & 64.8 & 79.0 \\
QExt-PLM+RC & MoCo & 18.6 & 44.0 & 26.5 & 28.6 & 44.8 & 15.5 & 32.3 & 15.0 & 24.6 & 12.1 & 53.0 & \secbestcell20.8 & 60.9 & 78.6 & 23.0 & 34.3 & 44.2 & 63.2 & 78.7 & 57.7 & 72.2 & 82.1 & 34.2 & 55.2 & 74.8 & 53.3 & 75.9 & 90.1 & 35.5 & 55.4 & 73.3 & 41.5 & 56.1 & 70.3 & 44.4 & 63.0 & 78.2 \\
 &  & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\

TQGen-Topic & Inbatch & 21.3 & 62.4 & \textbf{30.3} & 29.7 & 54.3 & 21.2 & 32.8 & 21.4 & \textbf{31.6} & 13.5 & 67.7 & 15.9 & 60.9 & 76.9 & 25.8 & \textbf{38.9} & 44.2 & 64.6 & 79.1 & 61.8 & 74.7 & 82.9 & 45.6 & 66.8 & 79.9 & 67.0 & 83.3 & 92.4 & 41.9 & 60.2 & 75.5 & 57.0 & 68.5 & 78.3 & 52.9 & 69.7 & 81.3 \\
TQGen-Topic+RC & Inbatch & 21.5 & 56.2 & 30.0 & 31.2 & 52.2 & 22.9 & 42.0 & 17.1 & 30.7 & 13.9 & 56.3 & 14.2 & 63.6 & 78.5 & 26.5 & 38.2 & 48.3 & 67.0 & 80.3 & 62.6 & 75.4 & 83.4 & 45.1 & 66.5 & 80.4 & 66.1 & 82.7 & 92.1 & 43.7 & 62.3 & 76.9 & 53.1 & 66.3 & 77.0 & 53.2 & 70.0 & 81.7 \\
TQGen-Topic & MoCo & 15.4 & 51.1 & 24.8 & 16.0 & 39.4 & 13.8 & 32.9 & 9.9 & 22.6 & 11.9 & 30.3 & 12.2 & 49.8 & 76.0 & 17.1 & 29.1 & 34.6 & 54.6 & 72.3 & 54.7 & 69.8 & 80.4 & 42.6 & 61.4 & 77.4 & 56.1 & 78.8 & 89.9 & 35.3 & 54.3 & 71.9 & 43.6 & 58.5 & 72.3 & 44.5 & 62.9 & 77.4 \\
TQGen-Topic+RC & MoCo & 21.3 & 62.1 & 27.6 & 29.9 & 53.9 & 20.8 & 39.2 & 18.9 & 29.8 & 13.8 & 55.7 & 15.1 & 64.5 & 80.2 & 25.5 & 38.3 & 46.4 & 66.5 & 80.5 & 63.8 & 76.0 & 83.6 & 47.3 & 67.7 & 80.8 & 68.6 & 84.2 & 93.2 & 44.5 & 63.6 & 78.6 & 53.8 & 66.9 & 77.9 & 54.1 & 70.8 & 82.4 \\
 &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

TQGen-Title & Inbatch & 20.8 & 58.6 & 30.1 & 31.0 & 52.0 & 22.6 & 32.0 & 20.4 & 30.4 & 14.2 & \bestcell\textbf{69.7} & 16.5 & 61.6 & 78.2 & 25.8 & 38.8 & 46.5 & 67.2 & 80.7 & 61.5 & 75.4 & 83.5 & 46.7 & 68.4 & 80.8 & 66.7 & 85.2 & 92.1 & 40.7 & 59.7 & 75.3 & 57.4 & 69.6 & 79.2 & 53.2 & 70.9 & 81.9 \\
TQGen-Title+RC & Inbatch & 20.9 & 49.3 & 28.8 & 30.7 & 45.1 & 22.7 & 39.7 & 13.7 & 28.2 & \textbf{14.4} & 58.6 & 15.0 & 64.2 & 77.3 & 25.8 & 36.7 & 48.5 & 68.0 & 81.0 & 63.0 & 75.8 & 83.6 & 45.9 & 68.3 & 80.9 & 68.3 & 85.5 & 91.9 & 42.6 & 61.6 & 76.6 & 53.7 & 67.1 & 77.7 & 53.6 & 71.0 & 82.0 \\
TQGen-Title & MoCo & 18.5 & 61.1 & 24.7 & 21.4 & 46.2 & 14.8 & 27.8 & 13.4 & 23.3 & 12.4 & 35.3 & 12.8 & 54.6 & 74.4 & 19.8 & 31.6 & 38.5 & 58.8 & 74.4 & 58.3 & 72.1 & 82.3 & 44.4 & 65.6 & 80.6 & 61.7 & 81.3 & 91.5 & 38.6 & 57.7 & 74.4 & 49.6 & 63.3 & 75.6 & 48.5 & 66.5 & 79.8 \\
TQGen-Title+RC & MoCo & 21.6 & 64.5 & 27.8 & 29.9 & 52.1 & 20.3 & 37.7 & \secbestcell\textbf{23.7} & 28.7 & 13.6 & 56.9 & 17.8 & 63.4 & 77.7 & 25.1 & 38.5 & 46.1 & 66.5 & 80.0 & 63.1 & 76.2 & 83.9 & 47.7 & 68.0 & 81.9 & 68.2 & 85.5 & 92.8 & 43.4 & 63.2 & 77.9 & 53.6 & 66.6 & 77.4 & 53.7 & 71.0 & 82.3 \\
 &  & & & & & & & & & & & & & & & &  & & & & & & & & & & & & & & & & & & &  &  &  \\

TQGen-AbSum & Inbatch & 17.4 & 51.2 & 27.7 & 27.2 & 46.8 & 20.8 & 35.3 & 15.5 & 26.5 & 14.1 & 64.0 & 16.1 & 60.5 & 77.8 & 25.3 & 36.3 & 47.2 & 67.1 & 81.1 & 63.4 & 76.4 & 83.9 & 48.8 & 69.6 & 81.6 & 68.9 & 86.3 & 93.2 & 42.5 & 60.9 & 76.6 & 57.6 & 69.7 & 79.5 & 54.7 & 71.7 & 82.6 \\
TQGen-AbSum+RC & Inbatch & 17.0 & 40.1 & 26.2 & 25.6 & 41.7 & 18.7 & 40.7 & 13.1 & 24.5 & 13.7 & 53.5 & 15.2 & 60.6 & 77.3 & 25.0 & 34.0 & 48.0 & 66.9 & 80.9 & 63.2 & 76.0 & 83.8 & 49.3 & 68.8 & 81.5 & 72.1 & 86.6 & 92.9 & 44.4 & 62.7 & 77.3 & 53.3 & 66.7 & 77.6 & 55.0 & 71.3 & 82.3 \\
TQGen-AbSum & MoCo & 21.2 & 53.3 & 25.3 & 25.9 & 45.6 & 17.3 & 41.2 & 15.7 & 24.7 & 13.6 & 40.5 & 15.7 & 59.8 & 71.0 & 21.2 & 33.6 & 46.1 & 65.9 & 79.4 & 63.8 & 75.9 & 83.9 & 50.5 & 69.6 & 81.5 & 70.9 & 85.7 & 92.9 & 44.3 & 63.3 & 78.3 & 52.5 & 66.3 & 78.1 & 54.7 & 71.1 & 82.4 \\
TQGen-AbSum+RC & MoCo & 21.2 & 61.3 & 25.5 & 31.0 & 52.2 & 19.7 & 38.2 & 20.1 & 27.4 & 13.4 & 56.0 & 19.1 & 61.5 & 73.0 & 22.4 & 37.2 & 47.5 & 67.2 & 80.7 & 64.5 & 76.5 & 84.0 & 49.5 & 68.5 & 81.0 & 69.5 & 85.7 & 93.1 & 44.2 & 63.3 & 78.1 & 54.7 & 67.6 & 78.2 & 55.0 & 71.5 & 82.5 \\
 &  & & & & & & & & & & & & & & & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\

TQGen-ExSum & Inbatch & 18.2 & 46.4 & 27.9 & 30.7 & 46.7 & 20.9 & 34.3 & 13.8 & 27.3 & 14.0 & 67.8 & 16.4 & 61.8 & 79.4 & \textbf{26.6} & 36.7 & 50.6 & 69.8 & 81.9 & 63.6 & 76.5 & 83.9 & 48.8 & 68.9 & 81.6 & 69.2 & 87.3 & 92.8 & 43.4 & 61.9 & 77.3 & 57.0 & 68.9 & 78.6 & 55.4 & 72.2 & 82.7 \\
TQGen-ExSum+RC & Inbatch & 17.6 & 38.0 & 26.5 & 26.1 & 39.1 & 20.1 & 40.0 & 13.0 & 25.0 & 13.3 & 53.9 & 13.7 & 60.9 & 79.2 & 25.6 & 33.9 & 50.7 & 68.6 & 81.1 & 63.5 & 76.0 & 84.0 & 48.9 & 68.5 & 80.6 & 71.0 & 87.2 & 92.7 & 44.8 & 63.5 & 77.7 & 49.8 & 63.5 & 75.5 & 54.8 & 71.2 & 81.9 \\
TQGen-ExSum & MoCo & 22.8 & 60.8 & 26.7 & 31.1 & 51.9 & 18.7 & 36.5 & 16.2 & 28.5 & 13.6 & 47.9 & 15.8 & \textbf{64.5} & 73.6 & 23.2 & 36.4 & 48.9 & 67.5 & 81.0 & 65.8 & 77.1 & 84.3 & 51.6 & 69.8 & 81.8 & 70.5 & 86.5 & 92.8 & 47.2 & 65.2 & 79.4 & 53.9 & 67.1 & 78.4 & 56.3 & 72.2 & 82.9 \\
TQGen-ExSum+RC & MoCo & 22.5 & 57.9 & 27.0 & 32.6 & 54.9 & 19.4 & 39.9 & 17.6 & 30.4 & 13.4 & 57.6 & 17.5 & 62.7 & 75.0 & 24.3 & 37.9 & 49.5 & 67.3 & 81.2 & 65.9 & 77.1 & 84.3 & 51.1 & 70.1 & 82.1 & 72.2 & 85.9 & 92.5 & 46.2 & 64.9 & 79.3 & 56.1 & 68.5 & 78.8 & 56.8 & 72.3 & 83.0 \\
\bottomrule
\end{tabular}



\end{adjustbox}

\caption{Scores for all of the experiments in this paper. For MS MARCO and BEIR datasets, we report the nDCG$@$10. For six open-domain QA datasets, we report the Recall$@$5/20/100. We highlight the \colorbox{BrickRed!35}{best} and \colorbox{RoyalBlue!15}{second best} in each column, and \textbf{best} in each group per column.}
\label{tab:giant}
\end{minipage}

\end{table*}





\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{0.7}
\small
% \footnotesize
% \tiny
\begin{tabular}{lcccccccccccccccc}
\toprule
                    & MM   & BEIR Avg (14) & trec-covid & nfcorpus & nq   & hotpotqa & fiqa & arguana & webis-touche2020 & dbpedia-entity & scidocs & fever & climate-fever & scifact & quora & cqadupstack \\
\midrule\midrule
BM25                & 22.8 & 43.0   & 65.6       & 32.5     & 32.9 & 60.3     & 23.6 & 31.5    & 36.7             & 31.3           & 15.8    & 75.3  & 21.3          & 66.5    & 78.9  & 29.9        \\
DPR                 & 35.4 & 36.8   & 57.5       & 21.0     & 39.8 & 37.1     & 27.4 & 41.4    & 20.8             & 23.6           & 10.7    & 58.9  & 17.6          & 47.5    & 84.2  & 28.1        \\
ANCE                & 38.8 & 40.5   & 65.4       & 23.7     & 44.6 & 45.6     & 29.5 & 41.5    & 24.0             & 28.1           & 12.2    & 66.9  & 19.8          & 50.7    & 85.2  & 29.6        \\
% GTR-base (110M)     & 42.0 & 44.1   & 53.9       & 30.8     & 49.5 & 53.5     & 34.9 & 51.1    & 20.5             & 34.7           & 14.9    & 66.0  & 24.1          & 60.0    & 88.1  & 35.7        \\
ColBERT             & 40.1 & 44.4   & 67.7       & 30.5     & 52.4 & 59.3     & 31.7 & 23.3    & 20.2             & 39.2           & 14.5    & 77.1  & 18.4          & 67.1    & 85.4  & 35.0        \\
SPAR$\dagger$          & 38.0 & 41.5   & 14.8       & 16.5     & 15.0 & 35.5     & 9.4  & 15.0    & 5.2              & 21.7           & 7.7     & 14.4  & 1.5           & 29.3    & 64.2  & 17.7        \\
Spider$\dagger$              & 24.8 & 19.1   & 53.3       & 31.1     & 46.1 & 50.5     & 29.3 & 47.5    & 16.6             & 34.3           & 16.2    & 56.7  & 18.8          & 51.2    & 85.3  & 29.2        \\
LaPraDor$\dagger$            & 38.9 & 40.4   & 59.9       & 28.6     & 43.0 & 59.4     & 25.5 & 32.4    & 24.1             & 34.7           & 14.2    & 71.6  & 19.3          & 60.8    & 80.0  & 27.5        \\
Condenser (Book\&Wiki)$\dagger$ & 38.7 & 40.9   & 56.9       & 28.6     & 46.3 & 50.0     & 25.4 & 43.0    & 17.1             & 35.0           & 13.8    & 68.6  & 22.7          & 54.1    & 84.8  & 26.1        \\
CoCondenser (MSMARCO)$\dagger$  & 40.8 & 42.9   & 66.3       & 31.8     & 46.4 & 50.9     & 29.8 & 43.6    & 20.4             & 35.9           & 14.2    & 66.2  & 23.1          & 56.7    & 85.6  & 29.1        \\
Contriever$\dagger$         & \bestcell 41.3 & \secbestcell 45.2   & 65.4       & 33.1     & 52.0 & 64.6     & 32.8 & 26.1    & 18.9             & 42.0           & 15.9    & 74.8  & 21.9          & 67.6    & 85.7  & 32.6        \\
\midrule
QGen-D2Q      & 39.6 & 43.9   & 68.3       & 31.6     & 49.8 & 58.2     & 29.7 & 27.0    & 19.8             & 38.7           & 14.6    & 70.0  & 23.6          & 65.9    & 85.1  & 31.7        \\
RandomCrop    & 38.4 & 42.4   & 67.9       & 31.1     & 47.3 & 57.1     & 29.4 & 23.5    & 16.0             & 38.0           & 13.8    & 70.2  & 20.7          & 63.8    & 84.5  & 30.4        \\
QExt-PLM            & 38.8 & 42.5   & 67.7       & 31.8     & 47.2 & 57.8     & 28.0 & 22.2    & 17.9             & 38.4           & 14.4    & 69.7  & 20.6          & 63.9    & 84.6  & 31.1        \\
TQGen-Topic         & 38.8 & 43.2   & 70.0       & 31.0     & 48.1 & 58.1     & 28.5 & 24.4    & 19.7             & 38.0           & 14.6    & 71.2  & 21.5          & 63.5    & 84.9  & 30.7        \\
TQGen-Title         & 38.8 & 43.2   & 70.0       & 31.0     & 48.1 & 58.1     & 28.5 & 24.4    & 19.7             & 38.0           & 14.6    & 71.2  & 21.5          & 63.5    & 84.9  & 30.7        \\
TQGen-AbSum         & 39.1 & 43.9   & 71.7       & 31.8     & 50.0 & 59.6     & 30.1 & 22.1    & 18.3             & 39.4           & 15.1    & 73.5  & 21.9          & 65.4    & 84.8  & 31.1        \\
TQGen-ExSum         & 38.8 & 43.1   & 72.3       & 31.2     & 47.2 & 57.6     & 29.7 & 25.7    & 18.0             & 39.0           & 14.2    & 69.8  & 19.0          & 64.0    & 84.9  & 30.7        \\
Hybrid-All          & 38.9 & 43.6   & 68.3       & 31.6     & 48.2 & 58.9     & 28.4 & 24.9    & 20.3             & 39.1           & 14.7    & 72.8  & 22.1          & 65.0    & 85.1  & 30.4        \\
Hybrid-TQGen+       & 40.3 & 44.7   & 69.2       & 32.9     & 50.8 & 61.3     & 30.9 & 26.2    & 19.7             & 39.8           & 15.8    & 72.1  & 22.1          & 66.5    & 85.8  & 32.5        \\
Hybrid-TQGen++      & \secbestcell 40.9 & \bestcell 45.8   & 74.0       & 35.2     & 51.4 & 63.3     & 31.9 & 24.9    & 20.1             & 40.7           & 15.6    & 72.4  & 23.5          & 68.7    & 86.2  & 33.3     \\  
\bottomrule

\end{tabular}
\caption{Detailed fine-tuning scores.}
\label{tab:giant-ft}

\end{table*}

